Satellite Selection for In-Band Coexistence of Dense LEO Networks

We study spectrum sharing between two dense low-earth orbit (LEO) satellite constellations, an incumbent primary system and a secondary system that must respect interference protection constraints on the primary system. In particular, we propose a secondary satellite selection framework and algorithm that maximizes capacity while guaranteeing that the time-average interference and absolute interference inflicted upon each primary ground user never exceeds specified thresholds. We solve this NP-hard constrained, combinatorial satellite selection problem through Lagrangian relaxation to decompose it into simpler problems which can then be solved through subgradient methods. A high-fidelity simulation is developed based on public FCC filings and technical specifications of the Starlink and Kuiper systems. We use this case study to illustrate the effectiveness of our approach and that explicit protection is indeed necessary for healthy coexistence. We further demonstrate that deep learning models can be used to predict the primary satellite system associations, which helps the secondary system avoid inflicting excessive interference and maximize its own capacity.

==> DigComm_notation.tex <==
%\def\SNR{\mathrm{SNR}}
%\def\SINR{\mathrm{SINR}}
%\def\SIR{\mathrm{SIR}}
%\def\MMSE   {\mbox{\scriptsize \sf MMSE}}
%\def\sir {\mbox{\scriptsize\sf SIR}}
%\def\snr {\mbox{\scriptsize\sf SNR}}
%\def\sinr {\mbox{\scriptsize\sf SINR}}

\usepackage{xspace}

% \newcommand{\numbeams}{\ensuremath{N_{\mathrm{B}}}\xspace}

\def\sinc{\mbox{\textrm sinc}}

\def\Es{\mathcal{E}_s}
\def\Eb{\mathcal{E}_b}
\def\E{\mathbb{E}}
\def\dd{\mathrm{d}}

\newcommand{\ea}{\stackrel{(\text{a})}{=}}
\newcommand{\eb}{\stackrel{(\text{b})}{=}}
\newcommand{\ec}{\stackrel{(\text{c})}{=}}
\newcommand{\ed}{\stackrel{(\text{d})}{=}}
\newcommand{\ee}{\stackrel{(\text{e})}{=}}
\newcommand{\ef}{\stackrel{(\text{f})}{=}}
\newcommand{\eg}{\stackrel{(\text{g})}{=}}
\newcommand{\eh}{\stackrel{(\text{h})}{=}}
\newcommand{\ei}{\stackrel{(\text{i})}{=}}

%\newcommand*\diff{\mathop{}\!\mathrm{d}}

% Bold lowercase
\def\bydef{:=}
\def\ba{{\mathbf{a}}}
\def\bb{{\mathbf{b}}}
\def\bc{{\mathbf{c}}}
\def\bd{{\mathbf{d}}}
\def\bee{{\mathbf{e}}}
\def\bff{{\mathbf{f}}}
\def\bg{{\mathbf{g}}}
\def\bh{{\mathbf{h}}}
\def\bi{{\mathbf{i}}}
\def\bj{{\mathbf{j}}}
\def\bk{{\mathbf{k}}}
\def\bl{{\mathbf{l}}}
\def\bm{{\mathbf{m}}}
\def\bn{{\mathbf{n}}}
\def\bo{{\mathbf{o}}}
\def\bp{{\mathbf{p}}}
\def\bq{{\mathbf{q}}}
\def\br{{\mathbf{r}}}
\def\bs{{\mathbf{s}}}
\def\bt{{\mathbf{t}}}
\def\bu{{\mathbf{u}}}
\def\bv{{\mathbf{v}}}
\def\bw{{\mathbf{w}}}
\def\bx{{\mathbf{x}}}
\def\by{{\mathbf{y}}}
\def\bz{{\mathbf{z}}}
\def\b0{{\mathbf{0}}}


% Bold capital letters
\def\bA{{\mathbf{A}}}
\def\bB{{\mathbf{B}}}
\def\bC{{\mathbf{C}}}
\def\bD{{\mathbf{D}}}
\def\bE{{\mathbf{E}}}
\def\bF{{\mathbf{F}}}
\def\bG{{\mathbf{G}}}
\def\bH{{\mathbf{H}}}
\def\bI{{\mathbf{I}}}
\def\bJ{{\mathbf{J}}}
\def\bK{{\mathbf{K}}}
\def\bL{{\mathbf{L}}}
\def\bM{{\mathbf{M}}}
\def\bN{{\mathbf{N}}}
\def\bO{{\mathbf{O}}}
\def\bP{{\mathbf{P}}}
\def\bQ{{\mathbf{Q}}}
\def\bR{{\mathbf{R}}}
\def\bS{{\mathbf{S}}}
\def\bT{{\mathbf{T}}}
\def\bU{{\mathbf{U}}}
\def\bV{{\mathbf{V}}}
\def\bW{{\mathbf{W}}}
\def\bX{{\mathbf{X}}}
\def\bY{{\mathbf{Y}}}
\def\bZ{{\mathbf{Z}}}

==> sec-methodology.tex <==
\section{Modeling Our Framework? }\label{sec:methodology}


This work focuses on enabling the secondary system to coexist with the incumbent primary system.
The coexistence mechanism we propose operates on top of the primary system's regular operations, meaning that the secondary system has no control over the primary system. Therefore, to ensure a realistic and practical analysis, we model key aspects of the primary system’s operations, including satellite-to-cluster associations and handover policies, based on the best available knowledge. Given that detailed operational data for Starlink is not publicly disclosed, we construct our primary system model using insights from our analysis and existing literature. By providing a well-founded methodology for modeling the primary system, we establish a credible foundation for evaluating coexistence strategies in real-world LEO satellite deployments.



\subsection{\leo Satellites}
To conduct a thorough and practically relevant analysis on the in-band coexistence of two dense \leo satellite communication systems at $20$ GHz, we consider two preeminent commercial systems mentioned in the introduction: Starlink by SpaceX and Project Kuiper by Amazon. We consider Starlink the primary and Kuiper the secondary system; this is motivated by the fact that Starlink has priority rights to the $19.7$--$20.2$~GHz band for downlink transmission. Indeed, based on current regulations, Kuiper is permitted to operate within that band along with Starlink with the understanding that it will not cause prohibitive interference to Starlink---coinciding with the analyses herein. 

We simulate the constellation of satellites in Starlink and Kuiper in a Walker-Delta fashion \cite{wd}, {realized using \textsc{Matlab}'s Aerospace Toolbox \cite{matlab}}, based on the orbital parameters detailed in \tabref{tab:spaceX} and \tabref{tab:kuiper}, which are extracted from public filings \cite{kuiper, spaceX_req}. The total numbers of primary and secondary satellites simulated in this work are $\nump=6900$ %\footnote{We consider Starlink's Gen1 satellites and part of Gen2 satellites.}
and $\nums=3236$.  


\begin{table}[t]
	\vspace{-0.25cm}
	\caption{SpaceX's Starlink Constellation Parameters \cite{spaceX_req}\cite{spaceXX}}
	\centering
	\label{tab:spaceX}
	\begin{tabular}{| c| c|c|c|c| }
		\hline
		% Alt. ($km$) & Inc. (${}^\circ$)  & $\mathrm{N_{pl}}$ & $\mathrm{N_{sat-pl}}$ & $\mathrm{N_{sat-total}}$  \\
		Altitude & Inclination &  Planes & Satellites/Plane & Total No.~Satellites \\
		\hline
		$540$ km & $ 53.2^\circ$ &$ 72$ & $22$& $1584$ \\
		\hline
		$550$ km & $ 53^\circ$ & $72$ & $22$ & $1584$ \\
		\hline 
		$560$ km & $97.6^\circ$ & $4$ & $43$ & $172$ \\
		\hline 
		$560$ km & $97.6^\circ$ & $6$ & $58$ & $348$ \\
		\hline
		$570$ km & $70^\circ$ &$ 36$ &$ 20$ &$ 720$ \\
		\hline
		$530$ km & $33^\circ$ & $28$ & $89$ & $2492$ \\
		\hline
	\end{tabular}
	\vspace{-0.3cm}
\end{table}

\begin{table}[t]
	\caption{Amazon's Project Kuiper Constellation Parameters \cite{kuiper}}
	\centering
	\label{tab:kuiper}
	\begin{tabular}{| c| c|c|c|c| }
		\hline
		Altitude & Inclination &  Planes & Satellites/Plane & Total No.~Satellites \\
		\hline
		$590$ km & $33^\circ$ & $28$ & $28$ &$ 784$ \\
		\hline 
		$610$ km & $42^\circ$ & $36$ & $36$ & $1296$ \\
		\hline 
		$630$ km & $51.9^\circ$ & $34$ & $34$& $1156$ \\
		\hline
	\end{tabular}
	%\vspace{-0.3cm}
\end{table}


%\subsection{Transmit and Receive Beams}




\subsection{Number of Cells a Satellite to Serve}


% \begin{figure}[t]
%     \vspace{-0.25cm}
% 	\centering	\includegraphics[width=\linewidth,height=0.24\textheight,keepaspectratio]{nn_fig/geomap_r}
% 	\caption{Geographical region considered in this work. This work focuses on ten clusters located within the red rectangular region, each assigned a unique priority. These clusters collectively comprise a total of 952 cells. }
% 	\label{fig:geo_map}
%     \vspace{-0.3cm}
% \end{figure}



The ground area of interest for our analysis is illustrated in \figref{fig:geo_map}. Based on our assessment, the number of ground cells a satellite must serve ranges from 80 to 110, with the potential to increase when considering larger coverage areas, consistent with findings in \cite{}. To model this, we assume that each cluster consists of $\numc=127$ cells, representing the number of cells a satellite serves within a short period. This results in a total of $\numg=10$ clusters within the region.
Each hexagon represents a cluster with an assigned priority shown in the figure, implying a form of prioritization in the order of satellite assignments. 
In other words, clusters may have different priorities based on factors such as the number of subscribers. For example, given the limited number of available satellites, denser areas may be prioritized to ensure higher service rates and better availability. 

\subsection{Interference Protection Constraint}
$\Delta T/T=6 \%$ maybe in Intro. Primary vs. Secondary, Co-primary. 

\subsection{Handover Policies}
%The satellite-to-cluster association depends on the handover policy adopted by the satellite systems. 
This work considers two widely used handover policies for the primary system: Highest Elevation (HE) and Maximum Contact Time (MCT) \cite{sat_handover}. Under the HE policy, a satellite system selects the satellite with the highest elevation angle relative to a specified area to serve that area. In particular, the handover period is set to 15 seconds when HE is implemented in the primary system, as observed in Starlink's operation \cite{starlink_measure}. In contrast, the MCT policy prioritizes the satellite that offers the longest contact time, thereby reducing the frequency of handovers and enhancing connection stability.

The satellite-to-cluster association is determined based on the selected handover policy and the predefined priority of clusters. Under the HE policy, if a satellite has the highest elevation relative to multiple ground clusters—a frequent scenario—the cluster with the highest priority is assigned to that satellite. Similarly, under the MCT policy, if a satellite provides the longest contact time across multiple clusters, it is associated with the cluster having the highest priority. After these primary assignments, satellites are subsequently allocated to other clusters based on the handover policy and cluster priority rankings.
To ensure consistency in our evaluation, we assume that the primary system maintains fixed cluster priorities and follows the same handover policies throughout the simulation duration. %This allows for a controlled analysis of the impact of different handover strategies on the satellite-to-cluster association and overall system performance.

\subsection{Primary Satellite-to-Cluster Associations}



==> sec-peer-review-title.tex <==
% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle
